Sequential Batch Learning in Finite-Action Linear Contextual Bandits

We study the sequential batch learning problem in linear contextual bandits with finite action sets, where the decision maker is constrained to split incoming individuals into (at most) a fixed number of batches and can only observe outcomes for the individuals within a batch at the batch's end. Compared with both standard online contextual-bandit learning and offline policy learning in contextual bandits, this sequential batch learning problem provides a finer-grained formulation of many personalized sequential decision making problems in practical applications, including medical treatment in clinical trials, product recommendation in e-commerce and adaptive experiment design in crowdsourcing. We study two settings of the problem: one where the contexts are arbitrarily generated and the other where the context vectors are mutually independent across actions and time and follow a common Gaussian distribution. In each setting, we establish a regret lower bound and provide an algorithm, whose regret upper bound nearly matches the lower bound. As an important insight revealed therefrom, in the former setting, we show that the number of batches required to achieve the fully online performance is polynomial in the time horizon, while for the latter setting, a pure-exploitation algorithm with a judicious batch partition scheme achieves the fully online performance even when the number of batches is less than logarithmic in the time horizon. In the stochastic context setting, we additionally provide tight margin-based (i.e. instance-dependent) upper and lower regret bounds that delineate performance in terms of how difficult the problem instance is. Together, our results provide a near-complete characterization of sequential decision making in linear contextual bandits when batch constraints are present.

==> problem_dependent.tex <==
\section{Problem-Dependent Regret Bounds}\label{sec:gap}

The regret bounds given in the previous two sections are problem-independent regret bounds (also known as gap-independent regret bounds in the bandits literature): they do not depend on the underlying parameters of the probability distribution. When the contexts are stochastic, under certain ``margin" conditions, we can also consider problem-dependent regret bounds that can result in sharper bounds than those problem-independent ones. When the number of contexts is small (e.g., $K=2$), there could be a large margin between the performance of the optimal context and any sub-optimal contexts if $\|\theta^\star\|_2$ is bounded away from zero, raising the possibility that a problem-dependent regret bound sometimes better than the worst-case regret $\Theta(\sqrt{dT})$ could be obtained in sequential batch learning. The next theorem characterizes this. 

\begin{theorem}\label{thm.problem-dependent}
	Assume $K=2$, and let $T$, $M=O(\log T)$, $d$ be the learning horizon, number of batches and the dimension of each context respectively. Denote by $\mathsf{polylog}(T)$ all the poly-logarithmic factors in $T$. Assume without loss of generality $\|\theta^*\|_2 > 0$. 
	\begin{enumerate}
		\item 
		Under Assumptions \ref{aspn.TKd} and \ref{assumption:cov}, there exists a sequential batch learning algorithm \textbf{Alg}= $(\calT, \pi)$ (explicitly defined below ) that achieves the following regret:
		\begin{align*}
	   \bE_{\theta^\star}[R_T(\pi)] \le \mathsf{polylog}(T)\cdot \frac{(d/\kappa)^{3/2}}{\|\theta^\star\|_2} \left(\frac{T}{d^2}\right)^{\frac{1}{M}}.
		\end{align*}
		\item
		Conversely, when the contexts $x_{t,a}\sim \calN(0,I_d/d)$ are independent over all $a\in [K], t\in [T]$, for any $M\le T$ and any sequential batch learning algorithm, we have:
		\begin{align*}
		\sup_{\theta^\star: \|\theta^\star\|_2\le 1} \|\theta^\star\|_2\cdot  \bE_{\theta^\star}[R_T(\pi)] \ge c\cdot d^{3/2} \left(\frac{T}{d^2}\right)^{\frac{1}{M}}, 
		\end{align*}
		where $c>0$ is a numerical constant independent of $(T,M,d)$. 
	\end{enumerate}
\end{theorem}
\begin{corollary}
In this setting, it is necessary and sufficient to have $\Theta(\log(T/d^2))$ batches to achieve the optimal problem-dependent regret $\tilde{\Theta}(d^{3/2} / \|\theta^\star\|_2)$. 
Here we are not aiming to get the tightest dependence on $\log T$ (note that $\tilde{\Theta}(\cdot)$ hides polylog factors). 
\end{corollary}

Note that the dependence on $T$ is significantly better than $\sqrt{T}$ in the problem-dependent bound, showing that a large $\|\theta^\star\|_2$ makes learning simpler. We remark that although the problem-dependent regret in Theorem \ref{thm.problem-dependent} only holds for $K=2$, the generalization to a generic $K$ is straightforward. Moreover, the margin between the optimal context and the sub-optimal context shrinks quickly as $K$ gets larger, and therefore the margin-based problem-dependent bound is not that useful compared with the worst-case regret bound in Theorem \ref{thm.stochastic} for large $K$. 

\subsection{Proof of the Upper Bound in Theorem \ref{thm.problem-dependent}}
The sequential batch learning algorithm which achieves the claimed upper bound is exactly the batched pure-exploitation algorithm with sample splitting shown in Algorithm \ref{algo.sample_splitting}, with a different choice of the grid: we consider a geometric grid $\calT' = \{t_1', t_2', \cdots, t_M'\}$ with
\begin{align*}
t_1' = bd^2, \qquad t_m' = \lfloor bt_{m-1}' \rfloor, \quad m=2,3,\cdots,M,
\end{align*}
where $b = \Theta((T/d^2)^{1/M})$ so that $t_M' = T$. Next we show that with the above choice of the grid, Algorithm \ref{algo.sample_splitting} attains the regret upper bound in Theorem \ref{thm.problem-dependent}. 

Consider the $m$-th batch with any $m\ge 2$, and any time point $t$ inside this batch. Define $v_t = x_{t,1} - x_{t,2}$, then our algorithm chooses the wrong arm if and only if $v_t^\top \theta^\star$ and $v_t^\top \hat{\theta}_{m-1}$ have different signs. Hence, the instantenous regret at time $t$ is
\begin{align*}
v_t^\top \theta^\star \cdot \mathbbm{1}(v_t^\top \theta^\star \ge 0, v_t^\top \hat{\theta}_{m-1} \le 0) - v_t^\top \theta^\star \cdot \mathbbm{1}(v_t^\top \theta^\star \le 0, v_t^\top \hat{\theta}_{m-1} \ge 0),
\end{align*}
and by the symmetry of $v_t\sim \calN(0,2\Sigma)$, it holds that
\begin{align*}
\bE\left[\max_{a\in \{1,2\}} (x_{t,a} - x_{t,a_t})^\top \theta^\star \right] = 2\bE\left[v_t^\top \theta^\star\cdot \mathbbm{1}(v_t^\top \theta^\star \ge 0, v_t^\top \hat{\theta}_{m-1} \le 0)  \right]. 
\end{align*}
Set $\delta = \sqrt{d\log T/(\kappa t_{m-1}')}$, and partition the non-negative axis $\bR_+$ into $\bigcup_{i=0}^\infty [i\delta, (i+1)\delta)$. Using this partition gives
\begin{align}
&\bE\left[v_t^\top \theta^\star\cdot \mathbbm{1}(v_t^\top \theta^\star \ge 0, v_t^\top \hat{\theta}_{m-1} \le 0)\cdot \mathbbm{1}(\|v_t\|_2 \le \sqrt{10\log T})  \right] \nonumber\\
&= \sum_{i=0}^\infty \bE\left[v_t^\top \theta^\star\cdot \mathbbm{1}(v_t^\top \theta^\star  \in [i\delta, (i+1)\delta), v_t^\top \hat{\theta}_{m-1} \le 0)\cdot \mathbbm{1}(\|v_t\|_2 \le \sqrt{10\log T}) \right] \nonumber\\
&\le \sum_{i=0}^\infty (i+1)\delta\cdot \bP\left(v_t^\top \theta^\star  \in [i\delta, (i+1)\delta), v_t^\top \hat{\theta}_{m-1} \le 0,\|v_t\|_2 \le \sqrt{10\log T} \right) \nonumber\\
&\le \sum_{i=0}^\infty (i+1)\delta\cdot \bP\left(v_t^\top \theta^\star  \in [i\delta, (i+1)\delta), v_t^\top (\theta^\star - \hat{\theta}_{m-1}) \ge i\delta,\|v_t\|_2 \le \sqrt{10\log T} \right) \nonumber\\
&\le \sum_{i=0}^\infty (i+1)\delta\cdot \bP\left(v_t^\top \theta^\star  \in [i\delta, (i+1)\delta) \right)\cdot \bP\left( v_t^\top (\theta^\star - \hat{\theta}_{m-1}) \ge i\delta \big| v_t^\top \theta^\star  \in [i\delta, (i+1)\delta), \|v_t\|_2 \le \sqrt{10\log T}\right). \label{eq.partition}
\end{align}

We deal with each term in \eqref{eq.partition} separately. For $\bP\left(v_t^\top \theta^\star  \in [i\delta, (i+1)\delta) \right)$, note that $v_t^\top\theta^\star$ is a normal random variable with variance $(\theta^\star)^\top \Sigma \theta^\star \ge \lambda_{\min}(\Sigma)\|\theta^\star\|_2^2\ge \kappa\|\theta^\star\|_2^2/d$, thus the probability density of this random variable is upper bounded by $\sqrt{d/2\pi \kappa}/\|\theta^\star\|_2$ everywhere. Therefore, 
\begin{align}\label{eq.anticoncentration}
\bP\left(v_t^\top \theta^\star  \in [i\delta, (i+1)\delta) \right) \le \delta\cdot \frac{\sqrt{d}}{\sqrt{2\pi\kappa}\|\theta^\star\|_2}. 
\end{align}
For the second term of \eqref{eq.partition}, the proof of Lemma \ref{lemma.difference} shows that the random vector $\theta^\star - \hat{\theta}_{m-1}\in \bR^d$ is $d/(c\kappa t_{m-1}')$-subGaussian for some absolute constant $c>0$, and is also independent of $v_t$. Hence, conditioning on $\|v_t\|_2\le \sqrt{10\log T}$, the random variable $v_t^\top(\theta^\star - \hat{\theta}_{m-1})$ is also subGaussian with parameter $\|v_t\|_2^2d/(c\kappa t_{m-1})\le 10d\log T/(c\kappa t_{m-1}')$. Consequently, subGaussian concentration gives
\begin{align}\label{eq.concentration}
\bP\left( v_t^\top (\theta^\star - \hat{\theta}_{m-1}) \ge i\delta \big| v_t^\top \theta^\star  \in [i\delta, (i+1)\delta), \|v_t\|_2 \le \sqrt{10\log T}\right) \le \exp\left(-\frac{c\kappa i^2\delta^2t_{m-1}'}{20d\log T}\right). 
\end{align}

Combining \eqref{eq.partition}, \eqref{eq.anticoncentration}, \eqref{eq.concentration} and the choice of $\delta$, we conclude that
\begin{align*}
\bE\left[v_t^\top \theta^\star\cdot \mathbbm{1}(v_t^\top \theta^\star \ge 0, v_t^\top \hat{\theta}_{m-1} \le 0)\cdot \mathbbm{1}(\|v_t\|_2 \le \sqrt{10\log T})  \right]  &\le \frac{d^{3/2}\log T}{\sqrt{2\pi \kappa^3}t_{m-1}'\|\theta^\star\|_2} \sum_{i=0}^\infty (i+1)e^{-ci^2/20} \\
&\le C\cdot \frac{d^{3/2}\log T}{\kappa^{3/2}t_{m-1}'\|\theta^\star\|_2}. 
\end{align*}
Moreover, since $v_t^\top \theta^\star \le 2$ almost surely and $\bP(\|v_t\|_2\ge \sqrt{10\log T})\le T^{-5}$, we also have
\begin{align*}
\bE\left[v_t^\top \theta^\star\cdot \mathbbm{1}(v_t^\top \theta^\star \ge 0, v_t^\top \hat{\theta}_{m-1} \le 0)\cdot \mathbbm{1}(\|v_t\|_2 > \sqrt{10\log T})  \right] \le 2T^{-5}. 
\end{align*}
Therefore, by the choice of the grid, the expected total regret in the $m$-th batch is at most
\begin{align*}
\left(C\cdot \frac{d^{3/2}\log T}{\kappa^{3/2}t_{m-1}'\|\theta^\star\|_2} + 2T^{-5}\right)\cdot t_m' = O\left(\frac{d^{3/2}\log T}{\kappa^{3/2}\|\theta^\star\|_2}\cdot \left(\frac{T}{d^2}\right)^{1/M} \right). 
\end{align*}

The first batch is handled in the same way as the upper bound proof of Theorem \ref{thm.stochastic}. Specifically, the expected total regret in the first batch is 
\begin{align*}
O\left( t_1'\cdot \sqrt{\frac{\log T}{d}} \right) = O\left(\sqrt{d^3\log T}\left(\frac{T}{d^2}\right)^{\frac{1}{M}}\right) = O\left(\frac{\sqrt{d^3\log T}}{\kappa^{3/2}\|\theta^\star\|_2}\left(\frac{T}{d^2}\right)^{\frac{1}{M}} \right).
\end{align*}
Finally summing up all batches $m=1,2,\cdots,M$ completes the proof. 

\subsection{Proof of the lower bound in Theorem \ref{thm.problem-dependent}} The proof is entirely analogous to the lower bound proof of Theorem \ref{thm.stochastic}. First we observe that by Lemma \ref{lemma.lower_bound}, for any $\Delta \in [0,1]$ and fixed grid $\calT = \{t_1, t_2, \cdots, t_M\}$ we have
\begin{align*}
\inf_\pi \sup_{\theta^\star: \|\theta^\star\|_2\le 1} \|\theta^\star\|_2\cdot  \bE_{\theta^\star}[R_T(\pi)] &\ge \Delta\cdot \inf_\pi \sup_{\theta^\star: \Delta\le \|\theta^\star\|_2\le 1} \bE_{\theta^\star}[R_T(\pi)] \\
&\ge \Delta^2 \cdot\sum_{m=1}^M \frac{t_m-t_{m-1}}{10\sqrt{d}}\exp\left(-\frac{16t_{m-1}\Delta^2}{d^2}\right). 
\end{align*}
Now define $s = \min\{m\in [M]: t_m \ge d^2 \}$, which always exists due to the assumption $T\ge d^2$. Choosing $\Delta \in \{1,d^2/t_s,d^2/t_{s+1},\cdots,d^2/t_M\} \subseteq [0,1]$ in the above inequality gives
\begin{align*}
\inf_\pi \sup_{\theta^\star: \|\theta^\star\|_2\le 1} \|\theta^\star\|_2\cdot  \bE_{\theta^\star}[R_T(\pi)] \ge c\cdot \max\left\{\frac{t_s}{\sqrt{d}}, \frac{d^{3/2}t_{s+1}}{t_s},  \frac{d^{3/2}t_{s+2}}{t_{s+1}},\cdots,  \frac{d^{3/2}T}{t_{M-1}} \right\}
\end{align*}
for some absolute constant $c>0$. Finally, applying $\max\{a_1,\cdots,a_n\} \ge \sqrt[n]{a_1a_2\cdots a_n}$ gives
\begin{align*}
\inf_{\pi} \sup_{\theta^\star: \|\theta^\star\|_2\le 1} \|\theta^\star\|_2\cdot  \bE_{\theta^\star}[R_T(\pi)] \ge c\cdot d^{3/2}\left(\frac{T}{d^2}\right)^{\frac{1}{M-s+1}} \ge c\cdot d^{3/2}\left(\frac{T}{d^2}\right)^{\frac{1}{M}},
\end{align*}
as claimed. 
